A Transformer-based Approach for Source Code Summarization

Generating a readable summary that describes the functionality of a program is known as source code summarization. In this task, learning code representation by modeling the pairwise relationship between code tokens to capture their long-range dependencies is crucial. To learn code representation for summarization, we explore the Transformer model that uses a self-attention mechanism and has shown to be effective in capturing long-range dependencies. In this work, we show that despite the approach is simple, it outperforms the state-of-the-art techniques by a significant margin. We perform extensive analysis and ablation studies that reveal several important findings, e.g., the absolute encoding of source code tokens' position hinders, while relative encoding significantly improves the summarization performance. We have made our code publicly available to facilitate future research.

==> table/old_examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
\centering
% \resizebox{\linewidth}{!}{%
\small
\begin{tabular}{ p{0.95\linewidth}}
\hline
\vspace{-5mm}
\begin{minted}[]{java}
private void removeOurUIs() {
    for (String uiName : UI_LIST) {
        uiDefaults.remove(uiName + STRING); 
    } 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: remove the ui delegate .\\
\vspace{-2mm}
{\color{blue} Full Model}: refreshes our ui delegate for the specified ui control type .\\
\vspace{-2mm}
{\color{blue} Human-written}: use our ui delegate for the specified ui control type .\\
\hline

% \vspace{-5mm}
% \begin{minted}[]{java}
% public Result Entry(NondominatedPopulation population, 
%                     TypedProperties properties) {
%     this(population, properties == null ? null : properties.getProperties()); 
% }
% \end{minted}
% \vspace{-2mm}
% {\color{blue} Base Model}: constructs a result file entry with the specified non - dominated population and properties . \\
% \vspace{-2mm}
% {\color{blue} Full Model}: constructs a result file entry with the specified non - dominated population and auxiliary properties .\\
% \vspace{-2mm}
% {\color{blue} Human-written}: constructs a result file entry with the specified non - dominated population and auxiliary properties .\\
% \hline

\vspace{-5mm}
\begin{minted}[]{java}
protected int read(InputStream inputStream,
                   byte[] buffer, char divider) 
                   throws IOException {
    int index = NUM ;
    do {
        byte readByte = (byte)(
            NUM & inputStream.read());
        if (readByte == -NUM || 
            readByte == (byte)divider) {
            return index ;
        }
        buffer[index] = readByte;
        index++ ;
    } while (index < buffer.length);
    return index; 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: reads a number of bytes from a given file reader until either read or divider or the buffer , the end ) .\\
\vspace{-2mm}
{\color{blue} Full Model}: reads bytes from a given file reader until either a specified character sequence is read , the buffer is completely filled or the end of file is reached .\\
\vspace{-2mm}
{\color{blue} Human-written}: reads bytes from a given file reader until either a certain character is read , the buffer is completely filled or the end of file is reached .\\
\hline

% Code: public void timing Event ( float fraction ) { current . x = ( int ) ( start . x + ( end . x - start . x ) * fraction ) ; current . y = ( int ) ( start . y + ( end . y - start . y ) * fraction ) ; track . set Car Position ( current ) ; }
% Ground Truth : ['timingtarget implementation : calculate and set the current car position based on the animation fraction']
% Base Model : ['timingtarget implementation : calculate and set the current car fraction based on the animation fraction']
% 81.53551038173114
% Full Model : ['timingtarget implementation : calculate and set the current car position based on the animation fraction']
% 100.0
% Full Better : True
\vspace{-5mm}
\begin{minted}[]{java}
public void timingEvent(float fraction) { 
    current.x = (int)(start.x + (end.x - start.x) * fraction);
    current.y = (int)(start.y + (end.y - start.y) * fraction);
    track.setCarPosition(current); 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: timingtarget implementation : calculate and set the current car fraction based on the animation fraction\\
\vspace{-2mm}
{\color{blue} Full Model}: timingtarget implementation : calculate and set the current car position based on the animation fraction\\
\vspace{-2mm}
{\color{blue} Human-written}: timingtarget implementation : calculate and set the current car position based on the animation fraction\\
\hline

% Code: public Buffered Header ( final Char Array Buffer buffer ) throws Parse Exception { super ( ) ; if ( buffer == null ) { throw new Illegal Argument Exception ( STRING ) ; } int colon = buffer . index Of ( STRING ) ; if ( colon == - NUM ) { throw new Parse Exception ( STRING + buffer . to String ( ) ) ; } String s = buffer . substring Trimmed ( NUM , colon ) ; if ( s . length ( ) == NUM ) { throw new Parse Exception ( STRING + buffer . to String ( ) ) ; } this . buffer = buffer ; this . name = s ; this . value Pos = colon + NUM ; }
% Ground Truth : ['creates a new header from a buffer . the name of the header will be parsed immediately , the value only if it is accessed .']
% Base Model : ['creates a new header from a buffer . the name of the name will be parsed immediately only if it only contains a parsed of the value only if it is accessed .']
% 62.256246927221994
% Full Model : ['creates a new header from a buffer . the name of the header will be parsed immediately , the value only if it is accessed . the name of the header cannot be accessed .']
% 73.8807405739135
% Full Better : True
\vspace{-5mm}
\begin{minted}[]{java}
public void filledEllipse(double x, double y, 
                          double semiMajorAxis, double semiMinorAxis) { 
    if(semiMajorAxis < NUM) 
        throw new IllegalArgumentException(STRING); 
    if(semiMinorAxis < NUM ) 
        throw new IllegalArgumentException(STRING); 
    double xs = scaleX(x); 
    double ys = scaleY(y); 
    double ws = factorX(NUM * semiMajorAxis); 
    double hs = factorY(NUM * semiMinorAxis); 
    if(ws <= NUM && hs <= NUM) 
        pixel(x, y); 
    else 
        offscreen.fill(
            new Ellipse2D.Double(xs - ws / NUM, ys - hs / NUM, ws, hs)); 
    draw(); 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: draws an filled square of given ellipse , centered on ( x , y ) .\\
\vspace{-2mm}
{\color{blue} Full Model}: draws an ellipse with given semimajor and semiminor axes , centered on ( x , y ) and semiminor axes and semiminor axes .\\
\vspace{-2mm}
{\color{blue} Human-written}: draws an ellipse with given semimajor and semiminor axes , centered on ( x , y ) .\\
\hline


\end{tabular}
% }
\caption{Qualitative examples showing the advantages of the ``Full Model'' over the ``Base Model''.}
\label{app:qual_example}
\end{table}



\begin{table}[ht]
\centering
% \resizebox{\linewidth}{!}{%
\small
\begin{tabular}{ p{0.95\linewidth}}
\hline
% Code: public void filled Ellipse ( double x , double y , double semi Major Axis , double semi Minor Axis ) { if ( semi Major Axis < NUM ) throw new Illegal Argument Exception ( STRING ) ; if ( semi Minor Axis < NUM ) throw new Illegal Argument Exception ( STRING ) ; double xs = scale X ( x ) ; double ys = scale Y ( y ) ; double ws = factor X ( NUM * semi Major Axis ) ; double hs = factor Y ( NUM * semi Minor Axis ) ; if ( ws <= NUM && hs <= NUM ) pixel ( x , y ) ; else offscreen . fill ( new Ellipse 2 D . Double ( xs - ws / NUM , ys - hs / NUM , ws , hs ) ) ; draw ( ) ; }
% Ground Truth : ['draws an ellipse with given semimajor and semiminor axes , centered on ( x , y ) .']
% Base Model : ['draws an filled square of given ellipse , centered on ( x , y ) .']
% 53.71494751791018
% Full Model : ['draws an ellipse with given semimajor and semiminor axes , centered on ( x , y ) and semiminor axes and semiminor axes .']
% 71.08500514766945
% Full Better : True


\vspace{-5mm}
\begin{minted}[]{java}
@Override public void paintComponent(Graphics g) { 
    super.paintComponent(g); 
    Graphics2D graphics = (Graphics2D) g; 
    graphics.setBackground(mColorSpectrumBackground); 
    RenderingHints renderHints = new RenderingHints(
                        RenderingHints.KEY_ANTIALIASING,
                        RenderingHints.VALUE_ANTIALIAS_ON); 
    renderHints.put(RenderingHints.KEY_RENDERING, 
                    RenderingHints.VALUE_RENDER_QUALITY); 
    graphics.setRenderingHints(render Hints); 
    drawFrequencies(graphics); 
    drawCursor(graphics); 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: renders the channel configs , lines , lines , and cursor\\
\vspace{-2mm}
{\color{blue} Full Model}: renders the channel configs , lines , labels , and cursor .\\
\vspace{-2mm}
{\color{blue} Human-written}: renders the channel configs , lines , labels , and cursor\\
\hline

% Code: public String choose Server Alias ( String key Type , Principal [ ] issuers , Socket socket ) { return default X 509 KM . choose Server Alias ( key Type , issuers , socket ) ; }
% Ground Truth : ['returns an alias to authenticate the server side of a secure socket given the public key type and the list of certificate issuer authorities recognized by the peer ( if any ) .']
% Base Model : ['choose an alias to authenticate the server side of a secure socket given the public key type and default list of certificate issuer authorities recognized by the peer .']
% 73.7646597488608
% Full Model : ['choose an alias to authenticate the client side of a secure socket given the public key type and the list of certificate issuer authorities recognized by the peer ( if any ) .']
% 89.01732118131125
% Full Better : True
\vspace{-5mm}
\begin{minted}[]{java}
public String chooseServerAlias(
                    String keyType, Principal[] issuers, Socket socket) { 
    return defaultX509KM.chooseServerAlias(keyType, issuers, socket); 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: choose an alias to authenticate the server side of a secure socket given the public key type and default list of certificate issuer authorities recognized by the peer .\\
\vspace{-2mm}
{\color{blue} Full Model}: choose an alias to authenticate the client side of a secure socket given the public key type and the list of certificate issuer authorities recognized by the peer ( if any ) .\\
\vspace{-2mm}
{\color{blue} Human-written}: returns an alias to authenticate the server side of a secure socket given the public key type and the list of certificate issuer authorities recognized by the peer ( if any ) .\\
\hline

% Code: static Windows File Attributes from Find Data ( long address ) { int file Attrs = unsafe . get Int ( address + OFFSETOF FIND DATA ATTRIBUTES ) ; long creation Time = unsafe . get Long ( address + OFFSETOF FIND DATA CREATETIME ) ; long last Access Time = unsafe . get Long ( address + OFFSETOF FIND DATA LASTACCESSTIME ) ; long last Write Time = unsafe . get Long ( address + OFFSETOF FIND DATA LASTWRITETIME ) ; long size = ( ( long ) ( unsafe . get Int ( address + OFFSETOF FIND DATA SIZEHIGH ) ) << NUM ) + ( unsafe . get Int ( address + OFFSETOF FIND DATA SIZELOW ) & NUM ) ; int reparse Tag = is Reparse Point ( file Attrs ) ? unsafe . get Int ( address + OFFSETOF FIND DATA RESERVED 0 ) : NUM ; return new Windows File Attributes ( file Attrs , creation Time , last Access Time , last Write Time , size , reparse Tag , NUM , NUM , NUM ) ; }
% Ground Truth : ['create a windowsfileattributes from a win32_find_data structure']
% Base Model : ['create a windowsfileattributes from the capture structure']
% 54.10822690539396
% Full Model : ['create a windowsfileattributes from a win32_file_attribute_data structure']
% 70.71067811865474
% Full Better : True
\vspace{-5mm}
\begin{minted}[]{java}
static WindowsFileAttributes fromFindData(long address) { 
    int fileAttrs = unsafe.getInt(address + OFFSETOF_FIND_DATA_ATTRIBUTES); 
    long creationTime = unsafe.getLong(address + OFFSETOF_FIND_DATA_CREATETIME); 
    long lastAccessTime = unsafe.getLong(address + OFFSETOF_FIND_DATA_LASTACCESSTIME); 
    long lastWriteTime = unsafe.getLong(address + OFFSETOF_FIND_DATA_LASTWRITETIME); 
    long size = ((long)(unsafe.getInt(address + OFFSETOF_FIND_DATA_SIZEHIGH)) << NUM) 
                + (unsafe.getInt(address + OFFSETOF_FIND_DATA_SIZELOW) & NUM); 
    int reparseTag = isReparsePoint(fileAttrs) ?
                     unsafe.getInt(address + OFFSETOF_FIND_DATA_RESERVED_0) : 
                     NUM;
    return new WindowsFileAttributes(
                fileAttrs, creationTime, lastAccessTime, lastWriteTime,
                size, reparseTag, NUM, NUM, NUM); 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: create a windowsfileattributes from the capture structure\\
\vspace{-2mm}
{\color{blue} Full Model}: create a windowsfileattributes from a win32\_file\_attribute\_data structure\\
\vspace{-2mm}
{\color{blue} Human-written}: create a windowsfileattributes from a win32\_find\_data structure\\
\hline

% Code: @ Override public void paint Component ( Graphics g ) { super . paint Component ( g ) ; Graphics 2 D graphics = ( Graphics 2 D ) g ; graphics . set Background ( m Color Spectrum Background ) ; Rendering Hints render Hints = new Rendering Hints ( Rendering Hints . KEY ANTIALIASING , Rendering Hints . VALUE ANTIALIAS ON ) ; render Hints . put ( Rendering Hints . KEY RENDERING , Rendering Hints . VALUE RENDER QUALITY ) ; graphics . set Rendering Hints ( render Hints ) ; draw Frequencies ( graphics ) ; draw Cursor ( graphics ) ; }
% Ground Truth : ['renders the channel configs , lines , labels , and cursor']
% Base Model : ['renders the channel configs , lines , lines , and cursor']
% 73.48889200874657
% Full Model : ['renders the channel configs , lines , labels , and cursor .']
% 91.2167909070388
% Full Better : True


\vspace{-5mm}
\begin{minted}[]{java}
public BufferedHeader(final CharArrayBuffer buffer) throws Parse Exception { 
    super(); 
    if(buffer == null) { 
        throw new IllegalArgumentException(STRING); 
    } 
    int colon = buffer.indexOf(STRING); 
    if(colon == -NUM) { 
        throw new ParseException(STRING + buffer.toString()); 
    } 
    String s = buffer.substringTrimmed(NUM, colon); 
    if(s.length() == NUM) { 
        throw new ParseException(STRING + buffer.toString()); 
    } 
    this.buffer = buffer; 
    this.name = s; 
    this.valuePos = colon + NUM; 
}
\end{minted}
\vspace{-2mm}
{\color{blue} Base Model}: creates a new header from a buffer . the name of the name will be parsed immediately only if it only contains a parsed of the value only if it is accessed .\\
\vspace{-2mm}
{\color{blue} Full Model}: creates a new header from a buffer . the name of the header will be parsed immediately , the value only if it is accessed . the name of the header cannot be accessed .\\
\vspace{-2mm}
{\color{blue} Human-written}: creates a new header from a buffer . the name of the header will be parsed immediately , the value only if it is accessed .\\
\hline

\end{tabular}
% }
\caption{Qualitative examples showing the advantages of the ``Full Model'' over the ``Base Model''.}
\label{app:qual_examples_2}
\end{table}

==> table/table2_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{%
\small
\begin{tabular}{l|c@{\hskip 0.125in} c@{\hskip 0.125in} c|c@{\hskip 0.125in} c@{\hskip 0.125in} c}
% \begin{tabular}{l|c c c|c c c}
\hline
\multirow{ 2}{*}{Methods} & \multicolumn{3}{c|}{Java} & \multicolumn{3}{c}{Python} \\ 
\cline{2-7}
& BLEU & METEOR & ROUGE-L & BLEU & METEOR & ROUGE-L \\ 
\hline
% \multicolumn{7}{l}{Prior Works} \\
% \hline
CODE-NN \cite{iyer2016summarizing} &  27.60 & 12.61 & 41.10 & 17.36 & 09.29 & 37.81 \\
Tree2Seq \cite{eriguchi2016tree} & 37.88 & 22.55 & 51.50 & 20.07 & 08.96 & 35.64 \\
RL+Hybrid2Seq \cite{wan2018improving} & 38.22 & 22.75 & 51.91 & 19.28 & 09.75 & 39.34 \\
DeepCom \cite{hu2018deep} & 39.75 & 23.06 &  52.67 & 20.78 & 09.98 & 37.35 \\
API+CODE \cite{hu2018summarizing} & 41.31 & 23.73 & 52.25 & 15.36 & 08.57 & 33.65 \\
Dual Model \cite{wei2019code} & 42.39 & 25.77 & 53.61 & 21.80 & 11.14 & 39.45 \\
\hline
% \multicolumn{7}{l}{This Work} \\
% \hline
Base Model & 43.41 & 25.91 & 52.71 & 31.02 & 18.24 & 44.22 \\
Full Model & {\bf 44.58} & {\bf 26.43} & {\bf 54.76} & {\bf 32.90} & {\bf 20.14} & {\bf 47.20} \\
\hline
\end{tabular}
}
\caption{Comparison of our proposed approach with the baseline methods. The results of the baseline methods are directly reported from \cite{wei2019code}.
The ``Base Model'' refers to the vanilla Transformer (uses absolute position representations) and the ``Full Model'' uses relative position representations and includes copy mechanism.}
% }
\label{table:results}
% \vspace{-2mm}
\end{table*}


==> table/table3.tex <==
*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{%
\small
\begin{tabular}{l|c@{\hskip 0.125in} c@{\hskip 0.125in} c|c@{\hskip 0.125in} c@{\hskip 0.125in} c}
% \begin{tabular}{l|c c c|c c c}
\hline
\multirow{ 2}{*}{Methods} & \multicolumn{3}{c|}{Java} & \multicolumn{3}{c}{Python} \\ 
\cline{2-7}
& BLEU & METEOR & ROUGE-L & BLEU & METEOR & ROUGE-L \\ 
\hline
Full model ($F_m$) & 44.58 & 26.43 & 54.76 & 32.90 & 20.14 & 47.20 \\
\hline
$F_m - $ Relative Position ($R_m$) & 44.26 & 26.23 & 53.58 & 31.58 & 18.76 & 45.05 \\
$F_m - $ Copy Attention ($C_m$) & 44.14 & 26.34 & 53.95 & 32.14 & 19.28 & 45.85 \\
% $F_m - $ Relative Position ($R_m$) & 44.26 (-0.32) & 26.23 (-0.20) & 53.58 (-1.18) & xx.xx & xx.xx & xx.xx \\
% $F_m - $ Copy Attention ($C_m$) & 44.14 (-0.44) & 26.34 (-0.09) & 53.95 (-0.81) & xx.xx & xx.xx & xx.xx \\
% $F_m - R_m - C_m$ &  43.41 (-1.17) & 25.91 (-0.52) & 52.71 (-2.05) & xx.xx & xx.xx & xx.xx \\
\hline
\end{tabular}
}
\caption{Ablation study on the principle components of the ``Full Model''.}
% }
\label{table:ablation_model}
% \vspace{-2mm}
\end{table*}




